On the Sample Complexity of Learning Sum-Product Networks

Sum-Product Networks (SPNs) can be regarded as a form of deep graphical models that compactly represent deeply factored and mixed distributions. An SPN is a rooted directed acyclic graph (DAG) consisting of a set of leaves (corresponding to base distributions), a set of sum nodes (which represent mixtures of their children distributions) and a set of product nodes (representing the products of its children distributions). In this work, we initiate the study of the sample complexity of PAC-learning the set of distributions that correspond to SPNs. We show that the sample complexity of learning tree structured SPNs with the usual type of leaves (i.e., Gaussian or discrete) grows at most linearly (up to logarithmic factors) with the number of parameters of the SPN. More specifically, we show that the class of distributions that corresponds to tree structured Gaussian SPNs with $k$ mixing weights and $e$ ($d$-dimensional Gaussian) leaves can be learned within Total Variation error $\epsilon$ using at most $\widetilde{O}(\frac{ed^2+k}{\epsilon^2})$ samples. A similar result holds for tree structured SPNs with discrete leaves. We obtain the upper bounds based on the recently proposed notion of distribution compression schemes. More specifically, we show that if a (base) class of distributions $\mathcal{F}$ admits an "efficient" compression, then the class of tree structured SPNs with leaves from $\mathcal{F}$ also admits an efficient compression.

==> reviews.tex <==
AISTATS 2020 REVIEWS: ACCEPTED!
Questions
1. [Summary] Please summarize the main claims/contributions of the paper in your own words.
This work studies the sample complexity of parameter learning of tree-shaped sum-product networks (SPNs).
The work utilises prior work on Gaussian mixture models to show that tree-shaped SPNs using d-dimensional leaves (Gaussians) with k mixing weights and e leaves can be learned within a total variation error (epsilon) of at most O( (ed^2+k)/epsilon2) samples.
The results is very interesting and relevant for the tractable probabilistic models community.
2. [Detailed Comments] Please enter a detailed review describing the strengths and weaknesses of the submission.
General remarks:
The paper seems very interesting but is rather difficult to read.
This is especially as the content of the paper is rather dense.
It would be helpful to have some more visual illustration guidance (if possible).
Further, I belief it should be state more clearly that this work is concerned with tree-shaped SPNs only.
This was only mentioned in a footnote and should be made more visible as the paper might otherwise be misleading to readers.

Strengths:
The paper explores an interesting approach which has been applied to Gaussian mixture and applied the so-called distribution learning framework onto SP.
For this purpose the authors introduce a signature representation of SPNs, which seems interesting, and proof their claims in a coherent way.

Weakness:
I belief some of the statements are unintentionally incorrect.

*) (page 1) "SPN can be specied by its graphical model which takes the form of a rooted tree"
This is generally not true. I urge the authors to make a clear distinction between SPNs and tree-shaped SPTs.
I can understand that it is necessary to examine the sub-set of tree-shaped SPNs (at least the definition of a path weight relies on this) but I would encourage the authors to not unintentionally confuse future readers by claiming that an SPNs is a tree.

*) (page 1) "SPNs can be considered a natural generalisation of mixture models"
I don't think this is true. SPNs are structured mixture models but not a natural generalisation, if anything a hierarchical mixture model would be a natural generalisation. I understand the intension behind this sentence, but I believe this is not quite correct.

*) (page 2) According to Ashtiani et al., the TV distance is defined as the supremum of the Lebesgue measurable subset of R^d. This paper, however, uses the Borel sigma-algebra which is more restricted than a Lebesgue measurable subset. I would recommend the authors clarify this.

Further, the math is sometimes hard to follow due to the heavy use of symbols.
I understand that the authors try to have a notation close to the paper of Ashtiani et al. but I feel that this might overcomplicate the notation at some points.
For example, as a reader familiar with the SPN literature I find the symbol for the structure of a SPN confusing at first.

Further minor comments are:
- (page 2) Defintion 1 and 2, maybe consider adding references to those definitions.
- (page 3) Definition 7 seems to indicate that a product distribution always fully factorises the domain. Is this intensionally? If so, why is this necessary?
- (page 3) Definition 9 is a bit confusing to read. Maybe introduce the symbols (x, +, ...) before-hand?
- (page 3) Definition 8 is not clear. The notation [n] was never introduced. Also what is |b| and why is it necessary that |b| = d, this seems wrong?
- (page 4) It should be noted that \tilde(O) notation hides certain factors. I'm not sure this was ever mentioned.
- (page 5) Please add references for Definition 13 & 14.
- (page 5) It is not clear why tau and t and m are now a function of epsilon.
- (page 6) What is X and N in Definition 18? This was never introduced.
- (page 6) I belief Definition 19 is only true for tree-shaped SPNs. This has to be made clear. (In general, there is no unique path to a leaf)

Regarding the related work: I would urge the authors to improve this section. Not all of the listed work is primarily focused on obtaining good results. For example [28] primarily focuses on a principled learning strategy and [22] primarily focuses on reducing the computational complexity of tree-shaped SPNs by merging similar sub-structures.

—-
I thank the authors for clarifying my questions.
3. [Score] Please provide an overall score for the submission.
Accept: Good paper
4. [Questions for the Authors] Please provide questions for authors to address during the author feedback period and point out which improvement would improve your score.
I'm willing to improve the score if the authors show that they will address the raised concerns.
5. [Review Summary] Please enter a 1-2 sentence summary of your review explaining your overall score.
The paper proposes an interesting and relevant piece of research for the SPN community but needs some further refinement.
I'm especially concerned that future readers unfamiliar with SPNs will become the false expectation that SPN are in fact trees, which is generally not the case.
Further, I believe that the paper needs some further improvements so that is easier to follow the idea and understand the paper.
6. [Reproducibility] Are the experiments (if present) detailed enough to allow reproducibility?
Not applicable.
7. [Code] Was the code made available by the authors?
No
8. [Expertise] Please rate your expertise on the topic of this submission.
Expert: Reviewer has published one or more papers on the exact setting of the submission.
9. [Confidence] Please rate your confidence in the score assigned.
Expert: Reviewer is absolutely certain.
Reviewer #2
Questions
1. [Summary] Please summarize the main claims/contributions of the paper in your own words.
This is an interesting paper about the estimation of sample complexity in SPNs. A tight (linear) upper bound for the tree-shaped case is provided for both the Gaussian and the discrete variable case. An interesting consequence of the result is not affect by the depth of the network, this supporting the use of deep SPNs.
2. [Detailed Comments] Please enter a detailed review describing the strengths and weaknesses of the submission.
The result sounds quite interesting and useful for people working in this area. The proofs are quite technical, but the authors makes relatively clear the derivation process. The paper do not provide empirical analysis, but this is probably not necessary for the kind of results reported here. The final part of the paper looks a bit hurried and deserves more clarification. Also a deeper discussion about the validity of the result for different kinds of SPNs (e.g., selective vs. non-selective) would be helpful.
3. [Score] Please provide an overall score for the submission.
Accept: Good paper
4. [Questions for the Authors] Please provide questions for authors to address during the author feedback period and point out which improvement would improve your score.
See S2.
5. [Review Summary] Please enter a 1-2 sentence summary of your review explaining your overall score.
An useful result for people working with SPN as it gives sample complexity and justifies the use of deep architectures.
6. [Reproducibility] Are the experiments (if present) detailed enough to allow reproducibility?
No experiments.
7. [Code] Was the code made available by the authors?
No
8. [Expertise] Please rate your expertise on the topic of this submission.
Medium: Reviewer is well-read on the topic, but has not published in it.
9. [Confidence] Please rate your confidence in the score assigned.
Medium: Reviewer has understood the main points in the paper, but skipped the proofs and technical details.
Reviewer #3
Questions
1. [Summary] Please summarize the main claims/contributions of the paper in your own words.
This paper shows that sum-product networks can be PAC-learned with sample complexity that is linear w.r.t. the number of edges and leaves of the network.
2. [Detailed Comments] Please enter a detailed review describing the strengths and weaknesses of the submission.
SPNs are a relatively new class of models and many aspects are still lacking theoretical understanding. Thus, sample complexity results for learning SPNs are welcome. So, assuming that the proofs are correct, this paper is worth publishing. (My competence in computational learning theory is limited so I was not able to assess correctness of the proofs.)
3. [Score] Please provide an overall score for the submission.
Accept: Good paper
4. [Questions for the Authors] Please provide questions for authors to address during the author feedback period and point out which improvement would improve your score.
None
5. [Review Summary] Please enter a 1-2 sentence summary of your review explaining your overall score.
The research question is well-motivated and the results seem sound.
6. [Reproducibility] Are the experiments (if present) detailed enough to allow reproducibility?
Not applicable
7. [Code] Was the code made available by the authors?
No
8. [Expertise] Please rate your expertise on the topic of this submission.
Medium: Reviewer is well-read on the topic, but has not published in it.
9. [Confidence] Please rate your confidence in the score assigned.
Medium: Reviewer has understood the main points in the paper, but skipped the proofs and technical details.

META REVIEW:

SPNs are a promising graphical model for which some theoretical results are still to be developed. This paper gives some sample complexity results for learning SPNs. The response from authors has resolved some doubts. It is important that the authors incorporate them in the paper (including perhaps a more specific abstract and even title, since the work is focused on trees).
